Second-order discretization of Dyson series: iterative method, numerical analysis and applications in open quantum systems

We propose a general strategy to discretize the Dyson series without applying direct numerical quadrature to high-dimensional integrals, and extend this framework to open quantum systems. The resulting discretization can also be interpreted as a Strang splitting combined with a Taylor expansion. Based on this formulation, we develop a numerically exact iterative method for simulation system-bath dynamics. We propose two numerical schemes, which are first-order and second-order in time step $\Delta t$ respectively. We perform a rigorous numerical analysis to establish the convergence orders of both schemes, proving that the global error decreases as $\mathcal{O}(\Delta t)$ and $\mathcal{O}(\Delta t^2)$ for the first- and second-order methods, respectively. In the second-order scheme, we can safely omitted most terms arising from the Strang splitting and Taylor expansion while maintaining second-order accuracy, leading to a substantial reduction in computational complexity. For the second-order method, we achieves a time complexity of $\mathcal{O}(M^3 2^{2K_{\max}} K_{\max}^2)$ and a space complexity of $\mathcal{O}(M^2 2^{2K_{\max}} K_{\max})$ where $M$ denotes the number of system levels and $K_{\max}$ the number of time steps within the memory length. Compared with existing methods, our approach requires substantially less memory and computational effort for multilevel systems ($M\geqslant 3$). Numerical experiments are carried out to illustrate the validity and efficiency of our method.

==> Dyson_series.tex <==
In this section, we introduce the general structure of open quantum systems and propose a second order discretization of the Dyson series \cite{dyson1949radiation} based on Strang splitting \cite{strang1968construction} and Taylor expansion.

% An open quantum system consists of two parts, the system of interest and a non-interesting environment (bath).
% In this paper, we refer to the system of interest as ``system.''
% The system of interest and the bath, as a whole, is referred as the ``combined system.''
% For the combined system, the time evolution of the density operator $\rho(t)$ follows the von Neumann equation
% \begin{equation}
% \label{eq_von_Neumann}
%     \dv{\rho(t)}{t} = -\ii [H,\rho(t)]
% \end{equation}
% where $H$ is the total Hamiltonian for the combined system.
% In general open quantum systems, the Hamiltonian can be represented as
% \begin{equation}
%     H = H_s \otimes \id_b + \id_s \otimes H_b + W_s\otimes W_b.
% \end{equation}
% In this Hamiltonian, $H_s$ is the Hamiltonian acting barely on the system state and $H_b$ is the Hamiltonian for the bath.
% The last term, $W_s\otimes W_b$, also denoted by $W$, refers to the interaction of the system and the bath, leading to quantum dissipation for the system part.
% In the interaction term $W$, $W_s$ acts on the system part and $W_b$ acts on the bath part.

% In this paper, we assume a bosonic bath initially in the thermal equilibrium, modeled by a large number of quantum harmonic oscillators.
% In this case, the bath Hamiltonian is given by
% \begin{equation}
%     H_b = \sum_{l=1}^L \frac{1}{2} \left(\hat{p}_l^2 + \omega_l^2\hat{q}_l^2\right)
% \end{equation}
% and $W_b$ in the interaction term $W$ is given by
% \begin{equation}
%     W_b = \sum_{l=1}^L c_l \hat{q}_l.
% \end{equation}
% The parameter $L$ is the number of quantum harmonic oscillators in the bath. The operators $\hat{p}_l$ and $\hat{q}_l$ are the momentum and position operators for the $l$th harmonic oscillator in the bath, respectively.
% $\omega_l$ is the frequency of the $l$th harmonic oscillator and $c_l$ is the coupling intensity between the system and the $l$th harmonic oscillator in the bath.
% In this paper, we assume that the bath is initially at the equilibrium state.
% The initial state of the combined system is given by
% \begin{equation}
%     \rho(0) = \rho_s(0) \otimes \rho_b(0)
%     = \rho_s(0) \otimes \frac{\exp(-\beta H_b)}{\tr\left(\exp(-\beta H_b)\right)}.
% \end{equation}
% In the equilibrium state of the bath $\rho_b(0)$, the parameter $\beta$ represents the inverse temperature.
% To obtain the reduced density operator for the system, we can trace out the bath degrees of freedom in the density operator of the combined system
% \begin{equation}
%     \rho_s(t) = \tr_b \left(\rho(t)\right).
% \end{equation}
% For a specific observable $O_s$ for the system, its expectation value can be given by
% \begin{equation}
%     \expval{O_s}(t) 
%     = \tr_s \left(
%         O_s \otimes \rho_s(t)
%     \right).
% \end{equation}
% In the rest part of this section, we formulate a discrete time expression for the computation of $\expval{O_s}(t)$, which turns out to be a discrete form of the Dyson series \cite{dyson1949radiation}.

% To start with, we write down the formal solution to \cref{eq_von_Neumann}, which is given by
% \begin{equation}
%     \rho(t) = \e^{-\ii H t} \rho(0) \e^{\ii H t}.
% \end{equation}
% With this formal solution, the expectation of $O_s$ is then given by
% \begin{equation}
% \begin{split}
%     \expval{O_s} &= \tr\left(
%         \rho(0) \e^{\ii H t} \left(O_s\otimes \id_b\right) \e^{-\ii H t}
%     \right) \\
%     & = \tr\left(
%         \rho(0) \left(\e^{\ii H \dt}\right)^n
%         \left(O_s \otimes \id_b \right)
%         \left(\e^{-\ii H \dt}\right)^n
%     \right) \\
%     & = \tr_s \left(
%         \rho_s(0) \tr_b \left(
%             \rho_b(0) \e^{\ii H t} O_s \e^{-\ii H t}
%         \right)
%     \right) \\
%     & = \tr_s\left(\rho_s(0) G(-n\dt,n\dt)\right)
% \end{split}
% \end{equation}
% if we assume $t$ being the multiple of time step $\Delta t$ and focus on the discrete time points where $t = 0,\dt, \cdots, N\dt$.
% In the expression, we use the notation 
% \begin{equation}
% \label{eq_full_propagator}
%     G(-t,t) = \tr_b\left(\rho_b(0)\e^{\ii H t} O_s \e^{-\ii H t}\right)
% \end{equation}
% for the full propagator \cite{cai2020inchworm,cai2023bold}.
% For simplicity of notation, we split the total Hamiltonian into two parts by $H=H_0 + W$ with $H_0 = H_s\otimes \id_b+\id_s\otimes H_b$ and $W = W_s \otimes W_b$.
% In this splitting, $H_0$ is regarded as an unperturbed Hamiltonian and the interaction term $W$ is regarded as a perturbation on the unperturbed Hamiltonian $H_0$.
% By applying the Strange splitting \cite{strang1968construction} to the exponential operator, the single step propagator is written as
% \begin{equation}
%     \e^{\pm \ii H \dt} = \e^{\pm \ii H_0 \dt/2} \e^{\pm \ii W \dt} \e^{\pm \ii H_0 \dt/2} + \mathcal{O}(\dt^3).
% \end{equation}
For the interaction operator $W$, we further apply second order Taylor expansion to its exponential operator
\begin{equation}
    \e^{\ii W\dt } \approx (\id \pm \ii W\dt - \frac{1}{2} W^2 \dt^2).
\end{equation}
Combining the Strang splitting and the Taylor expansion, we have
\begin{equation}
\begin{split}
    &\e^{\pm \ii H \dt} = \e^{\pm \ii H_0 \dt/2} \left(\id \pm \ii W \dt - \frac{1}{2}W^2 \dt^2\right) \e^{\pm \ii H_0 \dt/2} + \mathcal{O}(\dt^3) \\
    ={}& \e^{\pm \ii H_0 \dt}
    \pm \ii \e^{\pm \ii H_0 \dt/2}W\e^{\pm \ii H_0 \dt/2}\dt
    - \frac{1}{2}\e^{\pm \ii H_0 \dt/2} W^2 \e^{\pm \ii H_0 \dt/2} \dt^2 + \mathcal{O}(\dt^3).
\end{split}
\end{equation}
For simplicity of notation, we denote 
\begin{equation}
\label{eq_single_step_propagator}
\begin{split}
    &P_0 = \e^{-\ii H_0 \dt}, \\
    &P_1 = -\ii\dt \e^{-\ii H_0 \dt/2} W \e^{-\ii H_0 \dt/2}, \\
    &P_2 = -\frac{1}{2} \dt^2 \e^{-\ii H_0 \dt / 2} W^2  \e^{-\ii H_0 \dt / 2}
\end{split}
\end{equation}
as three types of propagators.
With these propagators, we have 
\begin{equation}
\begin{split}
    \e^{-\ii H \dt} &= P_0 + P_1 + P_2 + \mathcal{O}(\dt^3) \\
    \e^{\ii H \dt} &= P_0^\dagger + P_1^\dagger + P_2^\dagger +\mathcal{O}(\dt^3)
\end{split}
\end{equation}
Therefore, the $n$ step full propagator $G(-n\dt,n\dt)$ defined in \cref{eq_full_propagator} can be written as the following sum
\begin{equation}
\label{eq_full_propagator_expansion}
\begin{split}
    &G(-n\dt,n\dt) \\
    \approx &
    \sum_{k_1^\pm=0}^2
    \sum_{k_2^\pm=0}^2
    \cdots
    \sum_{k_{n-1}^\pm=0}^2
    \sum_{k_n^\pm=0}^2
    \tr_b \left(
        \rho_b(0)
         P_{k_n^-}^{\dagger}
         P_{k_{n-1}^-}^{\dagger}
         \cdots
         P_{k_2^-}^\dagger
         P_{k_1^-}^{\dagger}
         O_s 
         P_{k_1^+}
         P_{k_2^+}
         \cdots
         P_{k_{n-1}^+}
         P_{k_n^+}
    \right).
\end{split}
\end{equation}
For the unperturbed part $H_0$, its exponential operator can be simply decomposed as the system part and the bath part:
\begin{equation}
\label{eq_split_unperturbed_Hamiltonian}
    \e^{\pm \ii H_0 \dt/2} = \e^{\pm \ii H_s \dt / 2} \otimes \e^{\pm \ii H_b \dt /2}.
\end{equation}
Following \cref{eq_split_unperturbed_Hamiltonian} and $W=W_s\otimes W_b$, in \cref{eq_single_step_propagator}, all single time step propagators can be split into system and bath parts
\begin{equation}
\label{eq_propagators_system_and_bath}
\begin{split}
    &\mathcal{P}_{s,0} = \e^{-\ii H_s \dt}, \quad
    \mathcal{P}_{b,0} = \e^{-\ii H_b \dt}, \\
    &\mathcal{P}_{s,1} = -\ii\dt\e^{-\ii H_s \dt/2}
    W_s
    \e^{-\ii H_s \dt/2}, \quad
    \mathcal{P}_{b,1} = \e^{-\ii H_b \dt/2}
    W_b
    \e^{-\ii H_b \dt/2}, \\
    &\mathcal{P}_{s,2} = -\frac{1}{2}\dt^2\e^{-\ii H_s \dt/2}
    W_s^2
    \e^{-\ii H_s \dt/2}, \quad
    \mathcal{P}_{b,2} = 
    \e^{-\ii H_b \dt/2}
    W_b^2
    \e^{-\ii H_b \dt/2}
    , \\
    & P_0 = \mathcal{P}_{s,0} \otimes \mathcal{P}_{b,0}, \quad
    P_1 = \mathcal{P}_{s,1} \otimes \mathcal{P}_{b,1}, \quad
    P_2 = \mathcal{P}_{s,2} \otimes \mathcal{P}_{b,2}. 
\end{split}
\end{equation}
For simplicity, $\mathcal{P}_{s,0},\mathcal{P}_{s,1},\mathcal{P}_{s,2}$ is referred as a bare propagator, a single-interaction propagator and a double-interaction propagator, respectively, in the rest of this paper.
With the splitting of system and bath parts,
we can then split the full propagator \cref{eq_full_propagator_expansion} into system and bath parts:
\begin{equation}
\label{eq_full_propagator_system_bath_separation}
\begin{split}
    G(-n\dt,n\dt)
    = \sum_{k_1^\pm=0}^2
    \cdots
    \sum_{k_n^\pm=0}^2
    &
    \mathcal{P}_{s,k_n^-}^\dagger
    \cdots
    \mathcal{P}_{s,k_1^-}^\dagger
    O_s
    \mathcal{P}_{s,k_1^+}
    \cdots
    \mathcal{P}_{s,k_n^+} \\
    \times & \tr_b\left(
        \rho_b(0)
        \mathcal{P}_{b,k_n^-}^\dagger
        \cdots
        \mathcal{P}_{b,k_1^-}^\dagger
        \mathcal{P}_{b,k_1^+}
        \cdots
        \mathcal{P}_{b,k_n^+}
    \right) \\
    =\sum_{k_1^\pm=0}^2
    \cdots
    \sum_{k_n^\pm=0}^2
    & \mathcal{U}_n^{(0)}(k_1^\pm,\cdots,k_n^\pm)
    \mathcal{L}_b(k_1^\pm,\cdots,k_n^\pm).
\end{split}
\end{equation}
where $\mathcal{U}_n^{(0)}$ is propagator for the system and $\mathcal{L}_b$ is called the bath influence functional \cite{cai2020inchworm}.
Thanks to the Wick's theorem \cite{wick1950evaluation,chen2017inchwormITheory,cai2020inchworm}, the bath influence functional can be computed explicitly
\begin{equation}
    \mathcal{L}_b(k_1^\pm,\cdots,k_n^\pm)
    = \begin{dcases}
        0 ,&
        m=\sum_{j=1}^n \left( k_j^- + k_j^+\right) \text{~is odd}, \\
        \sum_{\mathfrak{q}\in\mathcal{Q}_m} \prod_{(i,j)\in\mathfrak{q}} B(s_i,s_j) ,&
        m=\sum_{j=1}^n \left(k_j^- + k_j^+\right) \text{~is even}.
    \end{dcases}
\end{equation}
$\mathcal{Q}_m$ is the set of all possible pairings of $m$ points \cite{cai2020inchworm,cai2022fast,cai2023bold}.
For example, 
\begin{equation}
    \mathcal{Q}_m = \begin{dcases}
        \{\{(1,2)\}\}, & \text{~if~} m = 2 \\
        \{\{(1,2),(3,4)\},\{(1,3),(2,4)\},\{(1,4),(2,3)\}\}, & \text{~if~} m = 4 \\
        \dots
    \end{dcases} 
\end{equation}
The sequence $\boldsymbol{s}$ is determined by the choose of $k_j^\pm$.
Specifically, $\boldsymbol{s}$ is an non-descending sequence that contains $k_j^+$ values of $-\left(j-\frac{1}{2}\right)$ and $k_j^-$ values of $\left(j-\frac{1}{2}\right)$.
For example, when $n = 3$ and $k_1^+ = 0, k_2^+ = 1, k_3^+ = 2, k_1^- = 2, k_2^- = 1, k_3^- = 0$, the sequence $\boldsymbol{s}$ is given by $\left(-\frac{5}{2}, -\frac{5}{2}, -\frac{3}{2}, \frac{1}{2} \frac{1}{2}, \frac{3}{2}\right)$.
In this example, $k_1^+ = 0$ and $k_3^-=0$ indicate the absence of $-\frac{1}{2}$ and $\frac{5}{2}$ in the sequence $\boldsymbol{s}$. 
$k_2^+ = 1$ and $k_2^- = 1$ mean that $-\frac{3}{2}$ and $\frac{3}{2}$ appear once in the sequence $\boldsymbol{s}$. 
The values $-\frac{5}{2}$ and $\frac{1}{2}$ appear twice because $k_3^+ = 2$ and $k_1^- = 2$.
In this example, the bath influence functional is
\begin{equation}
\begin{split}
    &\mathcal{L}_b([k_3^- = 0,k_2^- = 1,k_1^- = 2,k_1^+ = 0,k_2^+ = 1,k_3^+ = 2]) \\
    =& 2B(-5\dt/2,-5\dt/2) B(-3\dt/2,\dt/2) B(\dt/2,3\dt/2) \\
    +& B(-5\dt/2,-5\dt/2) B(-3\dt/2,3\dt/2) B(\dt/2,\dt/2) \\
    +& 4B(-5\dt/2,-3\dt/2) B(-5\dt/2,\dt/2) B(\dt/2,3\dt/2) \\
    +& 2B(-5\dt/2,-3\dt/2) B(-5\dt/2,3\dt/2) B(\dt/2,\dt/2) \\
    +& 2B(-5\dt/2,\dt/2) B(-5\dt/2,\dt/2) B(-3\dt/2,3\dt/2) \\
    +& 4B(-5\dt/2,\dt/2) B(-5\dt/2,3\dt/2) B(-3\dt/2,\dt/2).
\end{split}
\end{equation}
There are in principle 15 terms but identical terms appear due to the duplicate values in the sequence $\boldsymbol{s}$.

When $n=1$, the full propagator is given by
\begin{equation}
\begin{split}
    G(-\dt,\dt) &= 
    \mathcal{P}_{s,0}^\dagger \mathcal{P}_{s,0}
    + \mathcal{P}_{s,1}^\dagger \mathcal{P}_{s,1} B(-\dt/2, \dt/2) \\
    &+ \mathcal{P}_{s,0}^\dagger \mathcal{P}_{s,2}
    B(-\dt/2,-\dt/2)
    + \mathcal{P}_{s,2}^\dagger \mathcal{P}_{s,0}
    B(\dt/2,\dt/2) \\
    &+ 2\mathcal{P}_{s,2}^\dagger \mathcal{P}_{s,2} B(-\dt/2, \dt/2)B(-\dt/2, \dt/2) \\
    &+ \mathcal{P}_{s,2}^\dagger \mathcal{P}_{s,2}B(-\dt/2, -\dt/2)B(\dt/2, \dt/2).
\end{split}
\end{equation}
The full propagator $G(-n\dt,n\dt)$ can be also represented by diagrammatic equations.
For example, when $n=1$, we have
\input{diagrammatic_equation_1.tex}%
In the diagrammatic representation, a short interval may have 0,1,2 interaction operators, corresponding to $\mathcal{P}_{s,0},\mathcal{P}_{s,1},\mathcal{P}_{s,2}$ or their complex conjugates.
All interaction operators are paired by arcs. 
Each arc stands for a two-point correlation scalar function $B$.

In general, for the expansion of $G(-n\dt,n\dt)$, each diagram on the right satisfies the following conditions:
\begin{itemize}
    \item the diagram starts from $-n\dt$ and ends at $n\dt$;
    \item there may be 0,1,2 interaction operators at the middle of each subinterval;
    \item the total number of interaction operators $m$ is an even number;
    \item there are $m/2$ arcs pairing the $m$ interaction operators.
\end{itemize}

\Cref{eq_full_propagator_system_bath_separation} provides a second order discretization of the full propagator $G(-t,t)$.
It shares similar structure as QuAPI discretization \cite{makri1992improved}.
Nevertheless, they are essentially different, which will be clarified later in \textcolor{red}{cross ref...}
It can also be regarded as a special discretization of Dyson series \cite{dyson1949radiation,cai2020inchworm} if we merge all adjacent exponential operators the products of $\mathcal{P}_{s,0},\mathcal{P}_{s,1},\mathcal{P}_{s,2}$.
We will elaborate it later in \textcolor{red}{cross ref...}

==> Iterative_scheme_new.tex <==
Since the structure of full propagator \cref{eq_full_propagator_system_bath_separation} is similar to the reduced density matrix in the QuAPI method, we can design an iterative method accordingly.
The basic idea is to focus of the propagator on a specific range and extend the propagator iteratively.
Since the interactions within the short interval may be paired to those beyond the interval, we have to leave some ``open interactions'' to be connected with other interactions.

We start the algorithm from the observable in the middle of the expression and define $\Lambda_0 = O_s$.
Here, the subscript for $\Lambda$ stands for the time step.
$\Lambda_k$ represents the quantities within the range $[-k\dt,k\dt]$ and $\Lambda_{k+1/2}$ represents the quantities within the range $[(-k-1)\dt,k\dt]$.
Then we further extend $\Lambda_0$ by adding one of the three propagator $\mathcal{P}_{s,k}$ for $k=0,1,2$ respectively on the right side, which gives three different quantities:
\begin{equation}
\label{eq_half_step_propagator}
\begin{split}
    &\Lambda_{1/2}([0]) = \Lambda_0 \mathcal{P}_{s,0} + \Lambda_0 \mathcal{P}_{s,2} B(-\dt/2,-\dt/2),\\
    &\Lambda_{1/2}([1]) = \Lambda_0 \mathcal{P}_{s,1},\quad
    \Lambda_{1/2}([2]) = \Lambda_0 \mathcal{P}_{s,2}. 
\end{split}
\end{equation}
The parameter in the bracket stands for the number of interaction points to be connected on each small interval.
If we add a bare propagator $\mathcal{P}_{s,0}$ on the right of $\Lambda_0$, the resulting quantity will be a part of $\Lambda_{1/2}([0])$.
However, when we add a propagator $\mathcal{P}_{s,1}$, $\mathcal{P}_{s,2}$ without any arc, the resulting quantities becomes a part of $\Lambda_{1/2}([1])$ and $\Lambda_{1/2}([2])$ respectively.
However, if we add a double-interaction propagator and an arc connecting the two interactions, there will be no interaction waiting to be connected, so it becomes the second term in $\Lambda_{1/2}([0])$.

The next step is to add a propagator on the left of the quantities $\Lambda_{1/2}([k])$.
This step will give us the quantities of $\Lambda_1([k_1^-,k_1^+])$.
The parameter $k_1^+$ is the number of open interactions in the interval $[-\dt,0]$ and $k_1^-$ is the number of open interactions in the interval $[0,\dt]$.
There are many different cases in this step:
\begin{itemize}
    \item if we add a bare propagator on $\Lambda_{1/2}([0])$, it becomes a part of $\Lambda_{1}([0,0])$;
    \item if we add a single-interaction propagator on $\Lambda_{1/2}([0])$, it becomes a part of $\Lambda_{1}([1,0])$.
    \item if we add a double-interaction propagator on $\Lambda_{1/2}([0])$
    \begin{itemize}
        \item and no arc is added, it becomes a part of $\Lambda_{1/2}([2,0])$.
        \item and an arc is added to connect the two new interactions, it becomes a part of $\Lambda_1([0,0])$.
    \end{itemize}
    \item if we add a bare propagator on $\Lambda_{1/2}([1])$, it becomes a part of $\Lambda_{1}([0,1])$.
    \item if we add a single-interaction propagator on $\Lambda_{1/2}([1])$
    \begin{itemize}
        \item and no arc is added, it becomes a part of $\Lambda_{1/2}([1,1])$.
        \item and an arc connecting the new interaction and the existing interaction, it becomes a part of $\Lambda_1([0,0])$.
    \end{itemize}
    \item if we add a double-interaction propagator on $\Lambda_{1/2}([1])$
    \begin{itemize}
        \item and no arc is added, it becomes a part of $\Lambda_{1/2}([2,1])$.
        \item and an arc connecting to connect a new interaction and the existing interaction, it becomes a part of $\Lambda_1([1,0])$.
        \item and an arc connecting to connect two new interactions, it becomes a part of $\Lambda_1([0,1])$.
    \end{itemize}
    \item if we add a bare propagator on $\Lambda_{1/2}([2])$, it becomes a part of $\Lambda_{1}([0,2])$.
    \item if we add a single-interaction propagator on $\Lambda_{1/2}([2])$
    \begin{itemize}
        \item and no arc is added, it becomes a part of $\Lambda_{1}([1,2])$.
        \item and an arc is added to connected the new interaction and an existing interaction, it becomes a part of $\Lambda_{1}([0,1])$.
    \end{itemize}
    \item if we add a double-interaction propagator on $\Lambda_{1/2}([2])$
    \begin{itemize}
        \item and no arc is added, it becomes a part of $\Lambda_{1}([2,2])$.
        \item and an arc is added to connected a new interaction and an existing interaction, it becomes a part of $\Lambda_{1}([1,1])$.
        \item and an arc is added to connected two new interactions, it becomes a part of $\Lambda_{1}([0,2])$.
        \item and two arcs is added to connected the new interactions and the two existing interactions, it becomes a part of $\Lambda_{1}([0,0])$.
    \end{itemize}
\end{itemize}
We would like to point out that arcs are only allowed to added between two new interactions or between a new interaction and an existing interaction.
This prevents any diagrams to be double counted in the final summation.

Instead of defining $\Lambda_j$ for $j=1/2,1,2/3,\cdots$ directly based on $\Lambda_{j-1/2}$ directly like \cref{eq_half_step_propagator}, we use the strategy to extend the short one and add the results into its corresponding new quantity.
This process can be repeated for longer time simulation.
The order of the computation is 
\begin{equation}
    \Lambda_0 \Rightarrow \Lambda_{1/2}([k_1^+]) \Rightarrow \Lambda_1([k_1^\pm]) \Rightarrow \Lambda_{3/2}([k_1^\pm,k_2^+])
    \Rightarrow \Lambda_{2}([k_1^\pm,k_2^\pm]) 
    \Rightarrow \cdots.
\end{equation}
To compute $\Lambda_j$ for $j=1/2,1,3/2,\cdots$, we traverse all $\Lambda_{j-1/2}$'s from the last step, add one of the three propagators $\mathcal{P}_{s,k}$ on one side, add possible arcs, find the corresponding $\Lambda_{j}$ and add the newly computed quantity to $\Lambda_{j}$.
The reason to extend the short time propagators to longer time ones rather than obtaining the long time propagators by retrieving information from shorter time ones, is barely from the implementation's perspective.

Since the full propagator $G(-n\dt,n\dt)$ does not allow unconnected interactions, it is actually the quantity $\Lambda_n(\boldsymbol{0})$.
In other words, the method above allows efficient computation of the full propagator $G(-n\dt,n\dt)$ with extra cost of memorizing quantities $\Lambda_j(\boldsymbol{k})$ for all possible choices of $\boldsymbol{k}$.

Here, we would like to remark that this iterative process is actually a special resummation of the expansion \cref{eq_full_propagator_system_bath_separation}.
For a fixed $j$ and $\boldsymbol{k}$, the quantity $\Lambda_{j}(\boldsymbol{k})$ can be regarded as a part of \cref{eq_full_propagator_system_bath_separation}.
For each term in \cref{eq_full_propagator_system_bath_separation}, we only consider $j$ propagator on each side of $O_s$. 
The quantity $\boldsymbol{k}$, the quantity $\Lambda_{j}(\boldsymbol{k})$ is the sum of all diagrams whose unconnected interactions are given by $\boldsymbol{k}$.

==> iterative_scheme.tex <==
Inspired by the similarity of \cref{eq_full_propagator_system_bath_separation} and QuAPI, we design an iterative scheme for the computation of \cref{eq_full_propagator_system_bath_separation}.
The basic idea is to focus of the propagator on a specific range and extend the propagator iteratively.
Since the interactions within the short interval may be paired to those beyond the interval, we have to leave some ``open interactions'' to be connected with other interactions.

We first define the following three operators
\begin{equation}
    \mathcal{A}_0 = \e^{-\ii H_s \dt /2}, \quad
    \mathcal{A}_1 = -\ii\dt\e^{-\ii H_s \dt / 2} W_s, \quad
    \mathcal{A}_2 = -\frac{1}{2}\ii \dt W_s \e^{-\ii H_s \dt /2}.
\end{equation}
These three operators can be considered as three different half-step propagators.
The three system part single-step propagators $\mathcal{P}_{s,0},\mathcal{P}_{s,1},\mathcal{P}_{s,2}$ can be decomposed into half-step propagators by
\begin{equation}
    \mathcal{P}_{s,0} = \mathcal{A}_0 \mathcal{A}_0, \quad
    \mathcal{P}_{s,1} =  \mathcal{A}_1 \mathcal{A}_0, \quad
    \mathcal{P}_{s,2} = \mathcal{A}_1 \mathcal{A}_2.
\end{equation}
In the single-step propagators $\mathcal{P}_{s,0},\mathcal{P}_{s,1},\mathcal{P}_{s,2}$, we allow at most two interaction operators $W_s$ in the expression.
The three half-step propagators $\mathcal{A}_0,\mathcal{A}_1$ and $\mathcal{A}_2$ play the role as adding a half step bare propagator, adding the first interaction operator and adding the second interaction operator, respectively.

To better illustrate our idea, we first present our algorithm by first full step, which is further decomposed into four substeps.
The starting point of this iterative algorithm is the observable

\begin{itemize}
    \item Starting point
    \begin{equation}
        \Lambda_0(0) = O_s;
    \end{equation}
    \item propagate a half-step to the negative side
    \begin{equation}
        \Lambda_{1/4}^{(0)}(0) = \Lambda_0(0)\mathcal{A}_0, \quad
        \Lambda_{1/4}^{(1)}(1) = \Lambda_0(0) \mathcal{A}_1;
    \end{equation}
    \item Propagator another half-step to the negative side
    \begin{equation}
    \begin{split}
        &\Lambda_{2/4}(0) 
        = \Lambda_{1/4}^{(0)}(0) \mathcal{A}_0
        + \Lambda_{1/4}^{(1)}(1) \mathcal{A}_2 B(-\dt/2,-\dt/2), \\
        &\Lambda_{2/4}(1)
        = \Lambda_{1/4}^{(1)}(1) \mathcal{A}_0, \\
        &\Lambda_{2/4}(2) 
        = \Lambda_{1/4}^{(1)}(1) \mathcal{A}_2;
    \end{split}
    \end{equation}
    \item propagate a half-step to the positive side
    \begin{equation}
    \begin{split}
        &\Lambda_{3/4}^{(0)}([0,0]) 
        = \mathcal{A}_0^\dagger \Lambda_{2/4}(0), \\
        &\Lambda_{3/4}^{(1)}([0,0])
        = \mathcal{A}_1^\dagger \Lambda_{2/4}(1) B(-\dt/2,\dt/2) \\
        &\Lambda_{3/4}^{(0)}([0,1]) 
        = \mathcal{A}_0^\dagger \Lambda_{2/4}(1), \\
        &\Lambda_{3/4}^{(1)}([0,1]) 
        = \mathcal{A}_1^\dagger \Lambda_{2/4}(2) B(-\dt/2,\dt/2), \\
        &\Lambda_{3/4}^{(0)}([0,2]) 
        = \mathcal{A}_0^\dagger \Lambda_{2/4}(2), \\
        &\Lambda_{3/4}^{(1)}([1,0]) 
        = \mathcal{A}_1^\dagger \Lambda_{2/4}(0), \\
        &\Lambda_{3/4}^{(1)}([1,1]) 
        = \mathcal{A}_1^\dagger \Lambda_{2/4}(1), \\
        &\Lambda_{3/4}^{(1)}([1,2]) 
        = \mathcal{A}_1^\dagger \Lambda_{2/4}(2);
    \end{split}
    \end{equation}
    \item propagate another half-step to the positive side
    \begin{equation}
    \begin{split}
        \Lambda_1([0,0]) 
        =& \mathcal{A}_0^\dagger \Lambda_{3/4}^{(0)}([0,0])
        + \mathcal{A}_0^\dagger \Lambda_{3/4}^{(1)}([0,0]), \\
        +& \mathcal{A}_2^\dagger \Lambda_{3/4}^{(1)}([1,0]) B(\dt/2,\dt/2)
        + \mathcal{A}_2^\dagger \Lambda_{3/4}^{(1)}([0,1])
        B(-\dt/2,\dt/2), \\
        \Lambda_1([0,1])
        =& \mathcal{A}_0^\dagger \Lambda_{3/4}^{(0)}([0,1])
        + \mathcal{A}_0^\dagger \Lambda_{3/4}^{(1)}([0,1]) + \mathcal{A}_2^\dagger \Lambda_{3/4}^{(1)}([1,1]) B(\dt/2,\dt/2), \\
        \Lambda_1([0,2]) 
        =& \mathcal{A}_0^\dagger \Lambda_{3/4}^{(0)}([0,2]), \\
        \Lambda_1([1,0])
        =& \mathcal{A}_0^\dagger \Lambda_{3/4}^{(1)}([1,0]), \\
        \Lambda_1([1,1])
        =& \mathcal{A}_0^\dagger \Lambda_{3/4}^{(1)}([1,1]), \\
        \Lambda_1([1,2])
        =& \mathcal{A}_0^\dagger \Lambda_{3/4}^{(1)}([1,2]), \\
        \Lambda_1([2,0])
        =& \mathcal{A}_2^\dagger \Lambda_{3/4}^{(1)}([1,0]),\\
        \Lambda_1([2,1])
        =& \mathcal{A}_2^\dagger \Lambda_{3/4}^{(1)}([1,1]),\\
        \Lambda_1([2,2])
        =& \mathcal{A}_2^\dagger \Lambda_{3/4}^{(1)}([1,2]);
    \end{split}
    \end{equation}
    \item correction
    \begin{equation}
        \Lambda_1(0,0) \gets \Lambda_1(0,0) + \mathcal{A}_2^\dagger \mathcal{A}_1^\dagger\Lambda_{2/4}([0,2]) B(-\dt/2,\dt/2) B(-\dt/2,\dt/2)
    \end{equation}
\end{itemize}
The quantity $\Lambda_{1}([0,0])$ is actually the desired full propagator $G(-\dt,\dt)$.
The subscript of $\Lambda$ is the index for time, where each full time step is decomposed into four steps.


==> main_article.tex <==
% % SIAM Article Template
% \documentclass[review,hidelinks,onefignum,onetabnum]{siamart220329}

% % Information that is shared between the article and the supplement
% % (title and author information, macros, packages, etc.) goes into
% % ex_shared.tex. If there is no supplement, this file can be included
% % directly.

% \input{main_shared}

% % Optional PDF information
% \ifpdf
% \hypersetup{
%   % pdftitle={FRODS: the fast resummation of Dyson series},
%   pdftitle={Second-order discretization of Dyson series: iterative method, numerical analysis and applications in open quantum systems},
%   pdfauthor={authors}
% }
% \fi

% % The next statement enables references to information in the
% % supplement. See the xr-hyperref package for details.

% % \externaldocument[][nocite]{ex_supplement}

% % FundRef data to be entered by SIAM
% %<funding-group specific-use="FundRef">
% %<award-group>
% %<funding-source>
% %<named-content content-type="funder-name"> 
% %</named-content> 
% %<named-content content-type="funder-identifier"> 
% %</named-content>
% %</funding-source>
% %<award-id> </award-id>
% %</award-group>
% %</funding-group>

% \begin{document}

% \maketitle

% % REQUIRED
% \begin{abstract}
% We propose a general strategy to discretize the Dyson series without applying direct numerical quadrature to high-dimensional integrals, and extend this framework to open quantum systems. Based on this formulation, we develop a numerically exact iterative method for simulation system-bath dynamics. We propose two numerical schemes, which are first-order and second-order in time step $\Delta t$ respectively. We perform a rigorous numerical analysis to establish the convergence orders of both schemes, proving that the global error decreases as $\mathcal{O}(\Delta t)$ and $\mathcal{O}(\Delta t^2)$ for the first- and second-order methods, respectively. For the second-order method, we achieves a time complexity of $\mathcal{O}(M^3 2^{2K_{\max}} K_{\max}^2)$ and a space complexity of $\mathcal{O}(M^2 2^{2K_{\max}} K_{\max})$ where $M$ denotes the number of system levels and $K_{\max}$ the number of time steps within the memory length. Compared with existing methods, our approach requires substantially less memory and computational effort for multilevel systems ($M\geqslant 3$). Numerical experiments are carried out to illustrate the validity and efficiency of our method.
% \end{abstract}

% % REQUIRED
% \begin{keywords}
% Discrete Dyson series, open quantum systems, fast iterative method
% \end{keywords}

% % % REQUIRED
% % \begin{MSCcodes}
% % MSC codes here.
% % \end{MSCcodes}

% % \input{iterative_scheme}

% \section{Introduction}
% \label{sec_intro}
% \input{introduction.tex}

% \section{Discrete Dyson series}
% \label{sec_discrete_Dyson_series}
% \input{discrete_dyson}

% % \section{First order discretization of Dyson series}
% \section{Discrete Dyson series in open quantum systems}
% \label{sec_first_order}
% \input{first_order.tex}

% \section{Memory cost reduction}
% \label{sec_memory_cost_reduction}
% \input{memory_cost_reduction}

% \section{Proofs of convergence rates}
% \label{sec_proof}
% % \input{second_order}
% \input{second_order_new.tex}

% \section{Numerical results}
% \label{sec_numerical_result}
% \input{numerical_results}

% \section{Conclusion and future work}
% \label{sec_conclusion_and_future_work}
% \input{conclusion_and_future_work}

% \section{Appendix}
% \label{sec_appendix}
% \input{appendix}
% \bibliographystyle{siamplain}
% \bibliography{myBib_abbr}
% \end{document}


==> main_shared.tex <==
% % SIAM Shared Information Template
% % This is information that is shared between the main document and any
% % supplement. If no supplement is required, then this information can
% % be included directly in the main document.


% % Packages and macros go here
% \usepackage{lipsum}
% \usepackage{physics}
% \usepackage{amsfonts,amsmath,amssymb,mathrsfs}
% \usepackage{mathtools}
% \usepackage{graphicx}
% \usepackage{epstopdf}
% \usepackage{tikz}
% \usetikzlibrary{patterns,snakes,arrows.meta}
% \usepackage{algorithm}
% % \usepackage{algorithmic}
% \usepackage{algpseudocode}

% \usepackage{enumerate}
% \usepackage[shortlabels]{enumitem}
% % \usepackage{subfig}
% \usepackage{subcaption}
% \usepackage{tikz}
% \usepackage{diagbox}

% \usepackage{geometry}
% \geometry{left=2.5cm, right=2.5cm}

% \ifpdf
%   \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
% \else
%   \DeclareGraphicsExtensions{.eps}
% \fi

% % Add a serial/Oxford comma by default.
% \newcommand{\creflastconjunction}{, and~}

% % Used for creating new theorem and remark environments
% \newsiamremark{remark}{Remark}
% \newsiamremark{hypothesis}{Hypothesis}
% \crefname{hypothesis}{Hypothesis}{Hypotheses}
% \newsiamthm{claim}{Claim}
% \newsiamremark{RuleEnv}{Rule}
% \newsiamremark{RestrictionEnv}{Restriction}

% \newcommand{\dk}{\Delta k}
% \newcommand{\dt}{\Delta t}
% \newcommand{\e}{\mathrm{e}} % Euler's number e
% \newcommand{\id}{\mathrm{id}} % Identity operator
% \newcommand{\ii}{\mathrm{i}} % Imaginary unit, subscription i
% \newcommand{\ff}{\mathrm{f}}
% \newcommand{\sgn}{\mathrm{sgn}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\Ms}{\mathcal{M}}
% \newcommand{\bs}{\boldsymbol{s}}
% \newcommand{\Bcal}[2]{\mathcal{B}_{#1,#2}}
% \newcommand{\bk}{\boldsymbol{k}}
% \def\P{\mathbb{P}}
% \DeclareMathOperator{\SPAN}{span}
% \newcommand\added[1]{#1}
% \newcommand{\tensor}[1]{\underline{\mathbf{#1}}}
% \newcommand{\Pcal}{\mathcal{P}}

% \newcommand{\ki}[1]{\textcolor{orange}{[ki: #1]}}
% \newcommand{\zc}[1]{\textcolor{blue}{[ZC: #1]}}
% \newcommand{\yx}[1]{\textcolor{purple}{[yx: #1]}}
% \newcommand\dgm[2][.5]{\,\includegraphics[scale=#1]{figures/#2}\,}

% % Sets running headers as well as PDF title and authors
% % \headers{FRODS: the fast resummation of Dyson series}{Zhenning Cai, Yixiao Sun and Geshuo Wang}
% \headers{Second-Order Discretization of Dyson Series for Open Quantum Systems}{Zhenning Cai, Yixiao Sun and Geshuo Wang}

% % Title. If the supplement option is on, then "Supplementary Material"
% % is automatically inserted before the title.
% % \title{FRODS: the fast resummation of Dyson series}
% \title{Second-order discretization of Dyson series: iterative method, numerical analysis and applications in open quantum systems}

% % Authors: full names plus addresses.
% % \author{Zhenning Cai, Geshuo Wang}
% \author{Zhenning Cai\thanks{Department of Mathematics, National University of Singapore, 10 Lower Kent Ridge Road, Singapore 119076
%   (\email{matcz@nus.edu.sg}).}
% \and Yixiao Sun\thanks{Department of Mathematics, National University of Singapore, 10 Lower Kent Ridge Road, Singapore 119076
%   (\email{s.yixiao@u.nus.edu}).}
% \and Geshuo Wang\thanks{Department of Applied Mathematics, University of Washington, Seattle, WA 98195, USA
%   (\email{geshuo@uw.edu}).}}

% \usepackage{amsopn}
% \DeclareMathOperator{\diag}{diag}


% %%% Local Variables: 
% %%% mode:latex
% %%% TeX-master: "ex_article"
% %%% End: 


==> second_order.tex <==
The previous section answers the first question at the end of \cref{sec_first_order}.
In this section, we answer the second question by introducing a second order splitting.

In the iterative method we proposed in \cref{sec_first_order}, we apply Strang splitting and Taylor expansion for the exponential operatore $\e^{\pm \ii H\dt}$:
\begin{equation}
\begin{split}
    \e^{\pm \ii H \dt}
    &= \e^{\pm \ii H_0 \dt/2} \left(\id\pm\ii W \dt + \mathcal{O}(\dt^2)\right)\e^{\pm \ii H_0 \dt/2} + \mathcal{O}(\dt^3) \\
    &= \e^{\pm \ii H_0 \dt}
    \pm\ii\dt \e^{\pm \ii H_0 \dt/2}  W \e^{\pm \ii H_0 \dt/2}
    + \mathcal{O}(\dt^2)
\end{split}
\end{equation}
The discretization is locally of second order.
In numerical simulation, we compute the $n$ steps propagator $\left(\e^{\pm\ii H\dt}\right)^n$ where $n$ is proportional to $1/\dt$.
The power reduce the overall accuracy to first order.

In order to increase the convergence order, we have to include one more term in the Taylor expansion:
\begin{equation}
    \e^{\pm\ii W\dt}
    = \id \pm \ii W\dt - \frac{1}{2} W^2 \dt^2 + \mathcal{O}(\dt^3).
\end{equation}
Together with the Strang splitting, this expansion is locally of third order.
The overall convergence rate is of second order.

Following the idea in \cref{sec_first_order}, the only difference in the second order discretization is that each interval may now have 0,1 or 2 interactions.
There are three types of propagators with 0, 1 and 2 interaction operators respectively.
The first two propagators are given in \cref{eq_two_types_of_propagators}.
The extra propagator contains two interaction operators and is defined by
\begin{equation}
\begin{split}
    \mathcal{P}_{s,2} = -\frac{1}{2}\dt^2\e^{-\ii H_s \dt/2} 
    W^2
    \e^{-\ii H_s \dt/2} 
\end{split}
\end{equation}
This increases the number of diagrams as well as increase the memory cost.
In the first order scheme, there are only two diagrams in the expansion of $G(-\dt,\dt)$.
As a comparison, in the second order scheme, $G(-\dt,\dt)$ has the following diagrammatic expression:
\input{diagram_equation_G_dt_second_order}%
Since there may be 2 interaction operators at the same point, there exists some arcs connecting the same points or two arcs may have the same ending point.
Some diagrams may appear more than one time due to the same reason.

With the second order expansion, we can also derive an iterative method to compute $G(-n\dt,n\dt)$ based on the similar quantities $\Lambda_n(\bk)$.
We would like to point out some differences between the first order and the second order scheme.

The first obvious difference is that each component in $\bk$ has 3 possible choices rather than 2 choices in the first order method.
Therefore, the memory cost becomes $\mathcal{O}(3^{2n})$ for $\Lambda_n(\bk)$.
Even though we introduce the tricks proposed in \cref{sec_memory_cost_reduction}, the memory cost is still higher than the first order scheme.

The second difference is that for each propagation step, we may have at most four more interaction operators.
If we propagate both sides at the same time, a four nested loop is required.
Similar to what we mention in \cref{subsec_iterative_scheme}, if we propagate one side first and then the other side, we can convert the four nested loop to two double nested loops in a single time step.

Here, we would like to further reduce the computational cost by converting the double nested loops to single loops.
To decompose the double nested loops, we first introduce three types of half-step propagators:
\begin{equation}
\label{eq_half_step_propagators}
\begin{split}
    &\mathcal{H}_{s,0} = \e^{-\ii H_s \dt/2};\\
    &\mathcal{H}_{s,1} = -\ii \dt \e^{-\ii H_s \dt/2} W_s; \\
    &\mathcal{H}_{s,2} = -\frac{1}{2}\ii {\dt} W_s \e^{-\ii H_s \dt /2}.
\end{split}
\end{equation}
With these three half-step propagators, we have
\begin{equation}
\begin{split}
    &\mathcal{P}_{s,0} = \mathcal{H}_{s,0} \mathcal{H}_{s,0} \\
    &\mathcal{P}_{s,1} = \mathcal{H}_{s,1} \mathcal{H}_{s,0} \\
    &\mathcal{P}_{s,2} = \mathcal{H}_{s,1} \mathcal{H}_{s,2}
\end{split}
\end{equation}
In these half-step propagators \cref{eq_half_step_propagators}, there is at most one interaction in each propagator.
In other word, a single loop is required for a half-step propagator.
With this decomposition, the four nested loop is decoupled to four single loops.
This reduced the computational cost for the $n$th step from $\mathcal{O}(n^4 3^{2n})$ to $\mathcal{O}(n 3^{2n})$.
